Spatial Pricing of Ride-sourcing Services in a CongestedTransportation Network

We investigate the impacts of spatial pricing for ride-sourcing services in a Stackelberg framework considering traffic congestion. In the lower level, we use combined distribution and assignment approaches to explicitly capture the interactions between drivers' relocation, riders' mode choice, and all travelers' routing decisions. In the upper level, a single transportation network company (TNC) determines spatial pricing strategies to minimize imbalance in a two-sided market. We show the existence of the optimal pricing strategies for locational imbalance minimization, and propose effective algorithms with reliable convergence properties. Furthermore, the optimal pricing is unique and can be solved in a convex reformulation when matching time can be ignored. We conduct numerical experiments on different scales of transportation networks with different TNC objectives to generate policy insights on how spatial pricing could impact transportation systems.

==> Appendics/app_data.tex <==
% jd 2015-05-22 23:30
\section{Data inputs}\label{App:data_inputs}

\begin{table}[htbp]
  \centering
  \caption{Base Case Link Capacity $c_a$ (veh/h) and Free-flow Travel Time, FTT $t_a^0$ (min)}
  \resizebox{\columnwidth}{!}{
    \begin{tabular}{ccccccccccccccc}
    \toprule
    Link  & FFT   & Capacity  & \multicolumn{1}{c}{Link} & \multicolumn{1}{c}{FFT} & \multicolumn{1}{c}{Capacity } & \multicolumn{1}{c}{Link} & \multicolumn{1}{c}{FFT} & \multicolumn{1}{c}{Capacity } & \multicolumn{1}{c}{Link} & \multicolumn{1}{c}{FFT} & \multicolumn{1}{c}{Capacity } & \multicolumn{1}{c}{Link} & \multicolumn{1}{c}{FFT} & \multicolumn{1}{c}{Capacity } \\
    \midrule
1 & 12 & 777 & 17 & 6 & 235 & 32 & 10 & 300 & 47 & 10 & 151 & 62 & 12 & 152 \\
2 & 8 & 702 & 18 & 4 & 702 & 33 & 12 & 147 & 48 & 8 & 146 & 63 & 10 & 152 \\
3 & 12 & 777 & 19 & 4 & 147 & 34 & 8 & 146 & 49 & 4 & 157 & 64 & 12 & 152 \\
4 & 10 & 149 & 20 & 6 & 235 & 35 & 8 & 702 & 50 & 6 & 590 & 65 & 4 & 157 \\
5 & 8 & 702 & 21 & 20 & 151 & 36 & 12 & 147 & 51 & 16 & 150 & 66 & 6 & 146 \\
6 & 8 & 513 & 22 & 10 & 151 & 37 & 6 & 777 & 52 & 4 & 157 & 67 & 6 & 288 \\
7 & 8 & 702 & 23 & 10 & 300 & 38 & 6 & 777 & 53 & 4 & 145 & 68 & 10 & 152 \\
8 & 8 & 513 & 24 & 20 & 151 & 39 & 8 & 153 & 54 & 4 & 702 & 69 & 4 & 157 \\
9 & 4 & 533 & 25 & 6 & 417 & 40 & 8 & 146 & 55 & 6 & 590 & 70 & 8 & 150 \\
10 & 12 & 147 & 26 & 6 & 417 & 41 & 10 & 154 & 56 & 8 & 702 & 71 & 8 & 148 \\
11 & 4 & 533 & 27 & 10 & 300 & 42 & 8 & 148 & 57 & 6 & 437 & 72 & 8 & 150 \\
12 & 8 & 148 & 28 & 12 & 405 & 43 & 12 & 405 & 58 & 4 & 145 & 73 & 4 & 152 \\
13 & 10 & 300 & 29 & 8 & 146 & 44 & 10 & 154 & 59 & 8 & 150 & 74 & 8 & 153 \\
14 & 10 & 149 & 30 & 16 & 150 & 45 & 6 & 437 & 60 & 8 & 702 & 75 & 6 & 146 \\
15 & 8 & 148 & 31 & 12 & 147 & 46 & 6 & 288 & 61 & 8 & 150 & 76 & 4 & 152 \\
16 & 4 & 147 \\
    \bottomrule
    \end{tabular}%
    }
  \label{tab:capa_fft_base}%
\end{table}%


==> Appendics/app_derivatives.tex <==
% jd 2015-05-22 23:30
\chapter{Calculation of ${\partial \rho_{k'}}/{\partial g_i^j}$}\label{app: part_rho_part_g}

${\partial \rho_{k'}}/{\partial g_i^j}$ can be computed from the ISO's optimization problem (\ref{DP_ISO_nn_t}), where $\boldsymbol{\rho}$ is the dual variables of constraint (\ref{DP_ISO_fc2}) and $\boldsymbol{g}$ is parameters. ${\partial \rho_{k'}}/{\partial g_i^j}$ is essentially the derivative of dual variables with respect to right-hand side constants. We use the standard  notations for convex optimization with linear constraints:

\begin{subequations}\label{eq:stan_opti_nota}
\begin{alignat}{2}
\min_{\boldsymbol{x}}
&\phantom{===} \hspace{0.5cm} &&\phantom{=}f(\boldsymbol{x})   \label{stan_opti_of}\\
 \text{s.t.}
&\phantom{===} (\boldsymbol{\lambda}) &&\phantom{=}A\boldsymbol{x}=\boldsymbol{b}\label{stan_opti_cons}
\end{alignat}
\end{subequations}
 
\noindent where $f(\boldsymbol{x})$ is a convex function and $\boldsymbol{x} \in \mathbb{R}^n, \boldsymbol{\lambda}, \boldsymbol{b} \in \mathbb{R}^m$, to illustrate the calculating process and our goal is to calculate the Jacobian matrix $J_{\boldsymbol{\lambda}}(\boldsymbol{b})$.

Lagrangian of problem (\ref{eq:stan_opti_nota}) is $\mathcal{L} = f(\boldsymbol{x}) - \boldsymbol{\lambda}^{T}(A\boldsymbol{x}-\boldsymbol{b})$. The optimality conditions of problem (\ref{eq:stan_opti_nota}) is:

\begin{subequations}\label{eq:stan_opti_opti_cond}
\begin{align}
\nabla f(\boldsymbol{x}) - A^T\boldsymbol{\lambda} &= \boldsymbol{0}\label{stan_opti_opti_cond1}\\
A\boldsymbol{x}-\boldsymbol{b} &= \boldsymbol{0}\label{stan_opti_opti_cond2}
\end{align}
\end{subequations}

Take implicit derivatives of equations (\ref{eq:stan_opti_opti_cond}) with respect to $\boldsymbol{b}$ :

\begin{subequations}\label{eq:stan_opti_opti_cond_impl_deri}
\begin{align}
\nabla^2_{\boldsymbol{x}} f(\boldsymbol{x^{\ast}}(\boldsymbol{b})) J_{\boldsymbol{x}}(\boldsymbol{b}) - A^T J_{\boldsymbol{\lambda}}(\boldsymbol{b}) &= \boldsymbol{0}\label{stan_opti_opti_cond1_impl_deri}\\
AJ_{\boldsymbol{x}}(\boldsymbol{b})-\boldsymbol{I} &= \boldsymbol{0}\label{stan_opti_opti_cond2_impl_deri}
\end{align}
\end{subequations}

The unknown variables in equations (\ref{eq:stan_opti_opti_cond_impl_deri}) are two Jacobian matrices, $J_{\boldsymbol{x}}(\boldsymbol{b})$ and $J_{\boldsymbol{\lambda}}(\boldsymbol{b})$. The total number of equations is equal to the total number of variables in equations (\ref{eq:stan_opti_opti_cond_impl_deri}), which is $nm+m^2$. Therefore, in most cases, $J_{\boldsymbol{\lambda}}(\boldsymbol{b})$ can be calculated given $\boldsymbol{b}$. Numerically, one can take an initial guess of $\boldsymbol{b}$ based on historical data and then solve equations (\ref{eq:stan_opti_opti_cond_impl_deri}) and Algorithm \ref{alg: ph_trans} iteratively until $J_{\boldsymbol{\lambda}}(\boldsymbol{b})$ converged.






==> Appendics/app_flow.tex <==
\chapter{Small Example Illustrating Flow Conservation Constraint (\ref{DP_ISO_alf}) $\sim$ (\ref{DP_ISO_fc3})}\label{App:flow_exam}

\subsection*{Network Structure}
 \begin{figure}[htbp]
\begin{center}
    \includegraphics[width=0.4\textwidth]{./Figures/Energy/6node_network_structure.pdf}
\caption{Small Example Structure}
\label{fig:smal_exam_stru}
\end{center}
\end{figure}

\subsection*{OD and Path Information}
 \begin{table}[htbp]
 \caption{Small Example Structure}
 \vspace{-0.5cm}
\begin{center}
    \includegraphics[width=0.7\textwidth]{./Figures/Energy/od_path.pdf}
\label{fig:od_path}
\end{center}
\end{table}
\pagebreak
\subsection*{Network Flow}
 \begin{figure}[h]
\begin{center}
    \includegraphics[width=0.9\textwidth]{./Figures/Energy/network_flow.pdf}
\label{fig:netw_flow}
\caption*{}
\end{center}
\end{figure}
\vspace{-2cm}
\subsection*{Incidence Matrix}
 \begin{figure}[h]
\begin{center}
    \includegraphics[width=0.9\textwidth]{./Figures/Energy/incidence_matrix.pdf}
\label{fig:inci_matr}
\caption*{}
\end{center}
\end{figure}

